Shielded Deep Reinforcement Learning for Complex Spacecraft Tasking

Autonomous spacecraft control via Shielded Deep Reinforcement Learning (SDRL) has become a rapidly growing research area. However, the construction of shields and the definition of tasking remains informal, resulting in policies with no guarantees on safety and ambiguous goals for the RL agent. In this paper, we first explore the use of formal languages, namely Linear Temporal Logic (LTL), to formalize spacecraft tasks and safety requirements. We then define a manner in which to construct a reward function from a co-safe LTL specification automatically for effective training in SDRL framework. We also investigate methods for constructing a shield from a safe LTL specification for spacecraft applications and propose three designs that provide probabilistic guarantees. We show how these shields interact with different policies and the flexibility of the reward structure through several experiments.

==> sections/prelims.tex <==

\subsection{Specification Language}
We are interested in analyzing the temporal behavior of a satellite system w.r.t. a set of regions $R = \{r_1, \ldots, r_l\}$, where $r_i \subset \reals^n$. To this end, we define a set of atomic proposition $\Pi = \{\prop_1, \ldots, \prop_l\}$, where $\prop_i$ is true iff $\px \in r_i$ where $\px$ is the state of the satellite. Let $L: reals^n \to 2^\Pi$ be a labeling function that assigns to each state the set of atomic propositions that are true at that state. Then, an observation trace of trajectory $\omega_\px^N$ is $\rho = \rho_0 \rho_1 \ldots \rho_N$, where $\rho_i = L(\omega_\px^N(i))$ for all $0 \leq i \leq N$.  

To express the temporal properties of the system, we use LTLf~\cite{Giacomo2013}, which has the same syntax as LTL but its interpretations are over finite behaviors (traces).

\begin{definition}[LTLf]
    \label{def:LTLf}
    Given a set of atomic propositions $\Pi$, an LTLf formula is defined recursively as
    \begin{equation*}
        \varphi = \prop \mid \neg \varphi \mid \varphi \land \varphi \mid \bigcirc \varphi \mid  \varphi U \varphi  \mid F \varphi \mid G \varphi
    \end{equation*}
    where $\prop \in \Pi$, and $\bigcirc$, $U$, $F$, and $G$ are the ``next'', ``until'', "eventually", and "globally" temporal operators, respectively.
\end{definition}
The semantics of LTLf are defined over finite traces \cite{Giacomo2013}. We say a finite trajectory $\omega_\px$ satisfies formula $\varphi$, denoted by $\omega_\px \models \varphi$, if a prefix of its observation trace satisfies $\varphi$.



\subsection{Markov Models}

